IoT Connectivity Technologies and Applications: A Survey

The Internet of Things (IoT) is rapidly becoming an integral part of our life and also multiple industries. We expect to see the number of IoT connected devices explosively grows and will reach hundreds of billions during the next few years. To support such a massive connectivity, various wireless technologies are investigated. In this survey, we provide a broad view of the existing wireless IoT connectivity technologies and discuss several new emerging technologies and solutions that can be effectively used to enable massive connectivity for IoT. In particular, we categorize the existing wireless IoT connectivity technologies based on coverage range and review diverse types of connectivity technologies with different specifications. We also point out key technical challenges of the existing connectivity technologies for enabling massive IoT connectivity. To address the challenges, we further review and discuss some examples of promising technologies such as compressive sensing (CS) random access, non-orthogonal multiple access (NOMA), and massive multiple input multiple output (mMIMO) based random access that could be employed in future standards for supporting IoT connectivity. Finally, a classification of IoT applications is considered in terms of various service requirements. For each group of classified applications, we outline its suitable IoT connectivity options.

==> sections/3_section.tex <==
\newpage
\begin{table}[ht]
	%\scriptsize
	%\renewcommand{\arraystretch}{1.5}
	\begin{center}
	\caption{Difference to the Existing Survey Papers in the Areas of IoT/MTC}
	\begin{longtable}{|m{1.5cm}<{\centering}|m{3cm}<{\centering}|m{1.5cm}<{\centering}|m{1.5cm}<{\centering}|m{1cm}<{\centering}|m{1cm}<{\centering}|m{1.1cm}<{\centering}|m{1cm}<{\centering}|}
		%\hline\hlinem
		%\multicolumn{2}{|c|}  {\multirow{1}*{}}
		%\multicolumn{3}{|c|}{\multirow{1}*{}}
		%\\\hline
		\hline
		  \multirow{2}{*}{\textbf{Ref.}} & \multirow{2}{*} {\textbf{Main Focus}}  & \multicolumn{2}{m{3cm}<{\centering}|}{\textbf{Discussion on Existing Connectivity Technologies?}}& \multicolumn{4}{m{4cm}<{\centering}|}{\textbf{Overview of Emerging Technologies for Massive Connectivity?}} \\
		 \cline{3-8} 
		 &  & Short-range & Long-range & CS based & NOMA based & mMIMO based & ML based \\
		 	\hline
	     This Survey & State-of-the-art IoT connectivity technologies and their applications
       & \checkmark  &  \checkmark &  \checkmark  &  \checkmark  &  \checkmark  &  \checkmark \\
       	\hline
       \cite{Add_Survey1} & Cellular evolution challenges towards $5$G
       & $\times$  & $\times$ & $\times$  & $\times$  & $\times$  & $\times$ \\
       	\hline
       	\cite{Add_Survey2} & Spectrum sharing solutions for IoT connectivity 
       &  \checkmark  &  \checkmark & $\times$  & $\times$  & $\times$  & $\times$ \\
        \hline
       	\cite{Survey_comp5} & Short-range technologies and architectures for IoT
        &  \checkmark   & $\times$  & $\times$  & $\times$  & $\times$  & $\times$ \\
       	\hline
      	\cite{ Survey_comp6} & Comparison of Low-power technologies for IoT
        &  \checkmark   & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$ \\
       	\hline
       	\cite{Survey_comp1} &  IoT enabling technologies, protocols, and applications
       &  \checkmark &  $\times$  & $\times$  & $\times$  & $\times$  & $\times$ \\
       	\hline
       	\cite{wifi4} & Different LPWAN technologies and their applications
       &  \checkmark  &  \checkmark & $\times$  & $\times$  & $\times$  & $\times$ \\
        \hline
        \cite{ LPWAN3} &  LoRa for smart city applications
       &  \checkmark &  \checkmark  & $\times$  & $\times$  & $\times$  & $\times$ \\
       	\hline
       \cite{Add_Survey3} & LoRA, NB-IoT, and semantic web
       &  $\times$  &  \checkmark & $\times$  & $\times$  & $\times$  & $\times$ \\
        \hline
         
        \cite{Survey_comp7} & NB-IoT and its open issues
       &  $\times$  &  \checkmark & $\times$  & \checkmark  & $\times$  & $\times$ \\
        \hline
         
       	\cite{LPWAN2, Survey_comp2, LoraWAN2} & Comparison of different LPWAN from various perspectives
        &  $\times$  &  \checkmark  & $\times$  & $\times$  & $\times$  & $\times$ \\
       	\hline
       
       	\cite{ Survey_comp4} &  CS based IoT Applications
       &  $\times$ &  $\times$  & \checkmark  & $\times$  & $\times$  & $\times$ \\
       	\hline
       	\cite{NOMA1, NOMA2,Survey_comp3} & NOMA for massive IoT connectivity
       & $\times$  & $\times$ & $\times$  & \checkmark  & $\times$  & $\times$ \\
       	\hline
     	\cite{ mMIMO12} &  mMIMO for massive IoT connectivity
       &  $\times$ &  $\times$  & $\times$  & $\times$  & \checkmark  & $\times$ \\
       	\hline
       	\cite{ML14} &  ML based solutions for massive MTC
       &  $\times$ &  \checkmark  & $\times$  & $\times$  & $\times$  & \checkmark \\
       	\hline
	
	\end{longtable}
	\end{center}
\end{table}


==> sections/abstract.tex <==
\abstract{The Internet of Things (IoT) is rapidly becoming an integral part of our life and also multiple industries.
We expect to see the
number of IoT connected devices explosively grows and will reach hundreds of billions during the next few years.
To support such a massive connectivity, various wireless technologies are investigated. In this survey, we provide a broad view of the existing wireless IoT connectivity technologies and discuss several new emerging technologies and solutions that can be effectively used to enable massive connectivity for IoT. 
In particular, we categorize the existing wireless IoT connectivity technologies based on coverage range and review diverse types of connectivity technologies with different specifications. We also point out key technical challenges of the existing connectivity technologies for enabling massive IoT connectivity. To address the challenges, we further discuss
%In particular, we focus more on cellular IoT technologies as they can support massive connectivity for a large number of IoT devices in a wide area and discuss 
some examples of promising technologies such as compressive sensing (CS) random access, non-orthogonal multiple access (NOMA), and massive multiple input multiple output (mMIMO) based random access that could be employed in future standards for supporting IoT connectivity. 
%To help reader understand the essence of the connectivity technologies better, we explain and detail some key fundamental ideas and principle in the appendices. 
Finally, a classification of IoT applications is considered in terms of various service requirements. For each group of classified applications, we outline its suitable IoT connectivity options.}
